Hiding pebbles when the output alphabet is unary

Pebble transducers are nested two-way transducers which can drop marks (named "pebbles") on their input word. Blind transducers have been introduced by Nguy\^en et al. as a subclass of pebble transducers, which can nest two-way transducers but cannot drop pebbles on their input. In this paper, we study the classes of functions computed by pebble and blind transducers, when the output alphabet is unary. Our main result shows how to decide if a function computed by a pebble transducer can be computed by a blind transducer. We also provide characterizations of these classes in terms of Cauchy and Hadamard products, in the spirit of rational series. Furthermore, pumping-like characterizations of the functions computed by blind transducers are given.

==> parts/poubelle.tex <==
Let $A$ be an alphabet, $M$ be a finite monoid and $k \ge 0$.
We denote by $ \Cont_k(A,M) $ the set of elements of the
form $m_0 \cro{a_1}_{r_1} m_1 \cdots \cro{a_n}_{r_n} m_n $
where $m_0, \dots, m_n \in M$, $a_1, \dots, a_n \in A$ and $(r_1, \dots, r_n) \in \Sigma^+_k$.
Intuitively, it describes $n$ letters in a word from $A^*$, together with
some monoid elements abstracting the factors between these letters.
Furthermore, each letter is counted a certain number of times,
so that the total number of counts is $k$.

We now show by induction on $k \ge 1$ that given
a $k$-pebble bimachine $\mach = (A,M, \mu, \oras, \lambda)$, one can build a
$k$-machine which computes the same function.
Intuitively, the production on some $m_0 \cro{a_1}_{r_1} m_1 \cdots \cro{a_n}_{r_n} m_n$
will correspond to the sum of all productions
performed by the $k$-pebble bimachines when
marking $r_j$ times $a_j$ (with many possible orderings).



\begin{definition} \label{def:kmachine}
A \emph{$k$-machine} $\mach$ consists in:
\begin{itemize}
\item an input alphabet $A$;
\item a morphism into a finite monoid $\mu : A^* \rightarrow M$;
\item an output function $\prodd_{\mach} : \Cont_k(A,M) \rightarrow \Nat$.
\end{itemize}
\end{definition}






We only treat the case $k \ge 2$ and assume
by induction hypothesis that each $ \exte \in \oras$
can be computed by a $(k{-}1)$-machine $\nach_{\exte} = (\marq{A},N_{\exte}, \nu_{\exte}, \prodd_{\nach_{\exte}})$.
We define a $k$-machine $\nach = (A,N, \nu, \prodd_{\nach})$ which shall compute $f$ as follows:
\begin{itemize}
\item $\displaystyle N \defined M \times \prod_{\exte \in \oras} N_{\exte}$
and $\nu : w \mapsto (\mu(w), (\nu_{\exte}(w)_{\exte \in \oras})$;
\item let $m_0 \cro{a_1}_{r_1} m_1 \cdots \cro{a_n}_{r_n} m_n \in \Cont_k(A,N)$
(recall that $m_0, \dots, m_n {\in} M$, $a_1, \dots, a_n {\in} A$ and $(r_1, \dots, r_n) \in \Sigma^+_k$).
For $1 \le j \le n$, we define:
\begin{itemize}
\item $m_{j,\exte}$ (resp. $m_{j,M}$) the component
of $m_j$ in the monoid $N_{\exte}$ (resp. $M$);
\item  $\exte_j$ the function selected in $a_j$ by $\mach$, that is:
\begin{equation*}
\exte_j \defined \lambda(m_{0,M} \mu(a_1) \cdots m_{j{-}1,M},
a_j, m_{j{+}1,M} \mu(a_{j+1}) \cdots m_{n,M}) \in \oras;
\end{equation*}
\item $c_j \in \Cont_{{k}{-}1}(\marq{A},N_{\exte_j})$ as "the abstraction
seen when computing $\exte_j$ from letter $a_j$ by $\nach_{\exte_j}$",
that is (with the convention that $\cro{\marq{a_j}}_0 = \nu_{\exte_j}(\marq{a_j})$:
\begin{equation*}
c_j \defined  m_{0, \exte_j} \cro{a_1}_{r_1} m_{1, \exte_j} \cdots \cro{\marq{a_j}}_{r_j{-}1} m_{j+1, \exte_j}
\cro{a_j}_{r_j} \cdots m_{n, \exte_j};
\end{equation*}
 \end{itemize}
 Finally we define the production of $\mach$ as follows:
\begin{equation*}
\rod{\nach}{}{m_0 \cro{a_1}_{r_1} m_1 \cdots \cro{a_n}_{r_n} m_n}
\defined \sum_{j=1}^n  \rod{\nach_{\exte_j}}{}{c_j}.
\end{equation*}
\end{itemize}

The correctness of our construction is shown by the following:
\begin{claim}
For all $w \in A^*$, we have:
\begin{equation*}
fdsdfs
\end{equation*}
\end{claim}


\begin{definition}[Productions] We define by induction
on $\ell \ge 1$ the production $\rod{\trans}{w}{i_1, \dots, i_{\ell}}$
for $\trans$ a $\ell$-pebble bimachine, $w \in A^+$ and
$1 \le i_1, \dots, i_{\ell} \le |w|$:
\begin{itemize}
\item if $\ell = 1$, then $\trans = (A, \mu, \lambda,c)$ is a bimachine and we set:
\begin{equation*}
\rod{\trans}{w}{i_1} \defined \lambda(\mu(w[1{:}i_1{-}1]), w[i_1], \mu(w[i_1{+1}{:}|w|])).
\end{equation*}

\item if $\ell \ge 2$, then $\trans = (A, \mu, \lambda, \oras, c)$ is a bimachine with external pebble functions.
Let $\exte \defined \lambda(\mu(w[1{:}i_1{-}1]), w[i_1], \mu(w[i_1{+1}{:}|w|]) \in \oras$
and $\utrans$ be the $(\ell{-}1)$-pebble bimachine which computes $\exte \in \oras$.
We then define:
\begin{equation*}
\rod{\trans}{w}{(i_1, \dots, i_{\ell})} \defined \rod{\utrans}{\omar{w}{i_{1}}}{(i_2, \dots, i_{\ell})}.
\end{equation*}
\end{itemize}
\end{definition}

The function computed by the machine can easily be recovered
from its productions.

\begin{claim} \label{claim:sum-positions} If $\trans$ computes $f:A^* \rightarrow \Nat$,
then for all $w \in A^+$, we have:
\begin{equation*}
f(w) = \sum_{( i_1, \dots, i_k) \in [1{:}|w|]^k} \rod{\trans}{w}{(i_1, \dots, i_k)}.
\end{equation*}
\end{claim}












%%%% ANCIENNE PREUVE k-confusing


These productions can be easily decomposed and used to recover the output of $f$.
\begin{claim}
\label{claim:dec-prod}
If $m,n \in M$ and $w = w_1 \cdots w_{\ell}$ with $w_j \in A^*$, then:
\begin{equation*}
\pro{m\cro{w}n} = \sum_{j=1}^\ell \pro{m\mu(w_1 \cdots w_{j-1})\cro{w_j}\mu(w_{j+1}\cdots w_{\ell})n}.
\end{equation*}
In particular for $m,n$ neutral we get:
\begin{equation*}
f(w) = \sum_{j=1}^\ell \pro{\mu(w_1 \cdots w_{j-1})\cro{w_j}\mu(w_{j+1}\cdots w_{\ell})}.
\end{equation*}
\end{claim}



We can also note that the productions performed on iterations
of idempotents have a very simple shape, as detailed below.

\begin{claim} \label{claim:ct-idem}
If $m,n \in M$ and $u \in A^*$ is such that $\mu(u)$ is idempotent,
there exists a polynomial $P^{m,u,n} \in \Rel[X]$ of degree one
such that for all $X \ge 2$:
\begin{equation*}
\rod{\mach}{}{m \cro{u^{X}} n} = P(X)
\end{equation*}
\end{claim}


\begin{proof} Let $e \defined \mu(u)$, then for all $X \ge 2$ we have
by Claim \ref{claim:dec-prod}:
\begin{equation*}
\begin{aligned}
\rod{\mach}{}{m \cro{u^{X}} n} &= \rod{\mach}{}{m\cro{u u^{X-2} u} n} \\
&= \rod{\mach}{}{m\cro{u} e n}
+ \rod{\mach}{}{me\cro{u^{X-2}} e n} + \rod{\mach}{}{me\cro{u}n}
\\
& = \sum_{j=1}^{X-2} \rod{\mach}{}{me\cro{u} e n}
+ \rod{\mach}{}{m\cro{u} e n} + \rod{\mach}{}{me\cro{u}n}
\\
& = (X-2) \pro{me\cro{u} e n}
+ \rod{\mach}{}{m\cro{u} e n} + \rod{\mach}{}{me\cro{u}n}
\end{aligned}
\end{equation*}
which is a polynomial in $X$ of degree $1$ (the coefficients may not be non-negative).
\end{proof}





\begin{claim} \label{claim:final-confuse}
For all $m,n \in M$, there exists a polynomial
$Q \in \Rel[X_1, \dots, X_k]$ of degree $1$ such that
for all $X_1, \dots, X_k \ge 2$ we have:
\begin{equation*}
\rod{\mach}{}{m \cro{\alpha_0 \prod_{i=1}^k \tred{u_i}^{\omega X_i}\alpha_i} n}  = P(X_1, \dots, X_k)
\end{equation*}
\end{claim}

\begin{proof} We have by Claim \ref{claim:dec-prod}:
\begin{equation*}
\begin{aligned}
&\rod{\mach}{}{m \cro{\alpha_0 \prod_{i=1}^k \tred{u_i}^{\omega X_i}\alpha_i} n}\\
&= \sum_{j=0}^k \rod{\mach}{}{m \left(\prod_{i=0}^{j{-}1} \mu(\alpha_i) \tred{e_{i{+}1}}\right)
\cro{\alpha_j} \left(\prod_{i=j{+}1}^{k} \tred{e_i} \mu(\alpha_i)\right) n}\\
&+ \sum_{j=1}^k \rod{\mach}{}{m \left(\mu(\alpha_0)\prod_{i=1}^{j{-}1} \tred{e_i }\mu(\alpha_i) \right)
\cro{(\tred{u_j}^\omega)^{X_j}} \mu(\alpha_j) \left(\prod_{i=j{+}1}^{k} \tred{e_i} \mu(\alpha_i)\right) n}.
\end{aligned}
\end{equation*}
Since $e_j = \mu(u_j^\omega)$ is an idempotent, we can apply
Claim \ref{claim:ct-idem} to show that the $j$-th term of the second sum
is a polynomial of degree $1$ in $X_j$. Furthermore the first sum is a constant.
\end{proof}
 

Let $Q$ be the polynomial given by applying Claim \ref{claim:final-confuse}
to any of the two last terms of Equation \ref{eq:final-confuse}. 
It follows that for all $X_1, Y_1, \dots, X_k, Y_k \ge 2$ we have
for some $C \in \Nat$:
\begin{equation*}
\begin{aligned}
f(W(X_1, Y_1, \dots, X_k, Y_k))
&= Q(X_1, \dots, X_k) + Q(Y_1, \dots, Y_k) + C.
\end{aligned}
\end{equation*}

Since $Q$ is a polynomial of degree $1$, we finally
obtain the polynomial of Lemma \ref{lem:confuse-regular} by grouping the
terms of $X_i$ and $Y_i$ together.





















%%%% EXEMPLE DE FONCTION k-repetitive


\begin{example}
Given $a_1, \dots, a_{\ell} \in A$, the function $\cou{a_1, \dots, a_\ell} \defined \cou{a_1} \had \cdots \had \cou{a_\ell}$
from Example \ref{ex:count} is $k$-repetitive for all $k \ge 1$.
Let $\idem{} \defined 1$ and define some $W(X_1, Y_1, \dots, X_k, Y_k)$ as above.
Then for $1 \le j \le \ell$ there exists $C_j \ge 0$ such that:
\begin{equation*}
\begin{aligned}
\cou{a_j}(W(X_1, Y_1, \dots, X_k, Y_k)) &= C_j + \sum_{i=1}^{k}   \cou{a_j}( {u_i}) \omega (X_j + Y_j)
=: F_j[X_1+Y_1, \dots]
\end{aligned}
\end{equation*}
Then $F \defined \prod_{j=1}^\ell F_j$ is the function want for $\cou{a_1, \dots, a_\ell}$.
\end{example}














\section{Proof of Claim \ref{claim:sum-positions}}

Given an $k$-pebble bimachine $\trans$ 
which computes $f:A^* \rightarrow \Nat$, we show 
that for all $w \in A^+$:
\begin{equation*}
f(w) = \sum_{( i_1, \dots, i_k) \in [1{:}|w|]^k} \rod{\trans}{w}{(i_1, \dots, i_k)}.
\end{equation*}

The result is shown by induction on $k \ge 1$. If $k = 1$
then $\trans = (A, \mu, \lambda,c)$ and:
\begin{equation*}
f(w) = \sum_{1 \le i \le |w|} \lambda(w[1{:}i{-}1],w[i],w[i{+}1{:}|w|])
= \sum_{i \in [1{:}|w|]} \rod{\trans}{w}{i}.
\end{equation*}

If $k \ge 2$ then  $\trans = (A, \mu, \lambda, \oras, c)$ has external functions and:
\begin{equation*}
\begin{aligned}
f(w) & = \sum_{1 \le i \le |w|} \exte_{i}(\omar{w}{i}) \text{ where }
\exte_{i} \defined \lambda(\mu(w[1{:}{i{-}1}]),w[i],\mu(w[i{+}1{:}|w|]))\\
&=  \sum_{1 \le i \le |w|}  \sum_{(i_2, \dots, i_{k}) \in [1{:}|w|]^{k{-}1}}
\rod{\utrans_i}{\omar{w}{i}}{(i_2, \dots, i_{k})}
\text{ where } \utrans_i \text{ computes } \exte_{i}\\
& = \sum_{(i_1, \dots, i_{k}) \in [1{:}|w|]^{k}} \rod{\trans}{w}{(i_1, \dots, i_{k})}.
\end{aligned}
\end{equation*}















%%% PREUVE DU FACTEUR-COUPE pour r =1

 Let $e \defined \mu(u)$, then for all $X \ge 2$ we have:
\begin{equation*}
\begin{aligned}
\rod{\mach}{}{m \cro{u^{X}} n} &= \rod{\mach}{}{m\cro{u u^{X-2} u} n} \\
&= \rod{\mach}{}{m\cro{u} e n}
+ \rod{\mach}{}{me\cro{u^{X-2}} e n} + \rod{\mach}{}{me\cro{u}n}
\\
& = \sum_{j=1}^{X-2} \rod{\mach}{}{me\cro{u} e n}
+ \rod{\mach}{}{m\cro{u} e n} + \rod{\mach}{}{me\cro{u}n}
\\
& = (X-2) \rod{\mach}{}{me\cro{u} e n}
+ \rod{\mach}{}{m\cro{u} e n} + \rod{\mach}{}{me\cro{u}n}
\end{aligned}
\end{equation*}
which is a polynomial in $X$ of degree $1$ (some coefficients may be negative).
























\begin{itemize}
\item $\arch{\forest}{\{\nod_1, \dots, \nod_k\}} = 1$
\item if $\forest = \nod_1$ (then necessarily $k = 1$),
we set $\prune{\forest}{\forest} \defined w[\fr{\forest}{\forest}]$;
\item otherwise let $(\forest_1) \cdots (\forest_n) \defined \forest$.
For $1 \le j \le n$ we define $N_j \subseteq \{\nod_1, \dots, \nod_k\}$
for $1\le j \le n$ as the set of $\nod_i$ which
belong to $\forest_j$.
Then $ \biguplus_{1 \le j \le n} N_j = \{\nod_1, \dots, \nod_k\} $.
and we set:
\begin{equation*}
\begin{aligned}
\prune{\forest}{\{\nod_1, \dots, \nod_k\}}
&\defined t(\forest_1) \cdots t(\forest_n) 
 \text{ where:} \\
&t: \forest_j  \mapsto
\left\{
    \begin{array}{l}
        \displaystyle \left(\prune{\forest_j}{N_j}\right) \tnorm{ if } N_j \neq \varnothing;\\
        \tnorm{ otherwise} \left\{
   				 \begin{array}{l}
       				  \mu(\forest_j) \tnorm{ if } N_{j{-1}} \neq \varnothing \text{ or } N_{j{+1}} \neq \varnothing;\\
      				  \vide \tnorm{ otherwise.}\\
  				  \end{array}
				\right. \\
    \end{array}
\right.
\end{aligned}
\end{equation*}
\end{itemize}

















%%% PREUVE AVEC DES PRUNINGS



\section{Proof of Lemma~\ref{lem:pruning}}

Let $\mach$ be a $k$-marble bimachine
with morphism $\mu: A^* \rightarrow M$.
Let $w,w \in A^*$, $\forest \in \Fact{\mu}{w}$ $\forest' \in \Fact{\mu}{w'}$
and $\{\nod_1, \dots, \nod_k\} \in \Indeps{\forest}$ and 
$\{\nod'_1, \dots, \nod'_k\} \in \Indeps{\forest'}$.

We want to show that if:
\begin{equation*}
\prune{\forest}{\{\nod_1, \dots, \nod_k\}}  = \prune{\forest'}{\{\nod_1, \dots, \nod_k\}}
\end{equation*}
then:
\begin{equation*}
\rod{\mach}{\forest}{\{\nod_1, \dots, \nod_k\}} = \rod{\mach}{\forest'}{\{\nod'_1, \dots, \nod'_k\}}.
\end{equation*}


The intuition behind this result is that the positions
in the frontiers of $\nod_1, \dots, \nod_k$ or $\nod'_1, \dots, \nod'_k$
are in the same "context". Formally, we want to get the following:


We shall in fact show a more precise result:

\begin{definition} Given $1 \le j_1 < \dots < j_{\ell} \le |w|$,
we define the \emph{environnement}
\begin{equation*}
\env{w}{\mu}{\multi{j_1, \dots, j_{\ell}}} \defined \mu(w[1:j_1{-}1]) \cro{w[j_1]}  \mu(w[j_1{+}1{:}j_2{-}1])
\cdots \cro{w[j_{\ell}]}  \mu(w[j_{\ell}{+}1{:}|w|]).
\end{equation*}


\end{definition}

\begin{sublemma} \label{sub:biject-prod}
For all $1 \le i \le k$, there is a bjiection
$\sigma_i: \fr{\nod_i}{\forest} \rightarrow \fr{\nod'_i}{\forest'}$ such that
for all $j_1 \in \fr{\nod_1}{\forest}, \dots, j_k \in \fr{\nod_k}{\forest}$
\begin{equation*}
\env{w}{\mu}{\multi{j_1, \dots, j_k}} =  \env{w}{\mu}{\multi{\sigma(j_1), \dots, \sigma(j_k)}} 
\end{equation*}
\end{sublemma}

\begin{proof}[Proof of Lemma~\ref{lem:pruning} assuming Sublemma~\ref{sub:biject-prod}]
By definition of the semantics of a $k$-marble bimachine we have
for all $j_1 \in \fr{\nod_1}{\forest}, \dots, j_k \in \fr{\nod_k}{\forest}$:
\begin{equation*}
\rod{\forest}{\mach}{\multi{j_1, \dots, j_k}} =  \rod{\forest}{\mach}{\multi{\sigma(j_1), \dots, \sigma(j_k)}} 
\end{equation*}
and since:
\begin{equation*}
\rod{\forest}{\mach}{\multi{\nod_1, \dots, \nod_k}} = \sum_{j_i \in \fr{\nod_j}{\forest}}
\rod{\forest}{\mach}{\multi{j_1, \dots, j_k}} 
\end{equation*}
it suffices to apply the bijection to each term of the sum.
\end{proof}

The rest of this section is devoted to the proof of Sublemma~\ref{sub:biject-prod}.
Let $\mu: A^* \rightarrow M$ be defined as before,
the result is shown by induction on some $h \ge 1$.



\subparagraph*{Induction hypothesis on $h \ge 1$.}
Let $w,w \in A^*$, $\forest \in \Fact{\mu}{w}$ $\forest' \in \Fact{\mu}{w'}$,
both having height at most $h$, for all
$\{\nod_1, \dots, \nod_{\ell}\} \in \Indeps{\forest}$ and 
$\{\nod'_1, \dots, \nod'_{\ell}\} \in \Indeps{\forest'}$ if:
\begin{equation*}
\prune{\forest}{\{\nod_1, \dots, \nod_{\ell}\}}  = \prune{\forest'}{\{\nod'_1, \dots, \nod'_{\ell}\}}
\end{equation*}
then for all $1 \le i \le {\ell}$, there is a bijection
$\sigma_i: \fr{\nod_i}{\forest} \rightarrow \fr{\nod'_i}{\forest'}$ such that
for all $\{j_1, \dots, j_{\ell} \} \in \fr{\{\nod_1, \dots, \nod_k\}}{\forest}$:
\begin{equation*}
\env{w}{\mu}{\multi{j_1, \dots, j_{\ell}}} =  \env{w}{\mu}{\multi{\sigma(j_1), \dots, \sigma(j_{\ell})}} .
\end{equation*}


\subparagraph*{Base case $h = 1$.}
\gd{Horrible mais on y arrive.}

We show by induction on $h \ge 1$
that for all $\mu: A^* \rightarrow M$ morphism,
for all $k \ge 1$,  for all $k$-pebble bimachine $\trans$  with essential 
morphism $\mu$, for all $w \in A^+$,
for all $\forest \in \facto{\mu}{w}$ of height at most $h$,
we have the following:
\\
if $s \defined \{\nod_1, \dots, \nod_k\} \in \Indeps{\forest}$,
then $\rod{\forest}{\trans}{s}$ only depends on
$\prune{\forest}{s}$.

\subparagraph*{Proof.}
The proof of the induction case goes over
that of the base case, hence we focus on the induction case.
Let $h \ge 2$ and $\mu$, $k$, $w$, $\forest$ defined accordingly.

Let $s \defined \{\nod_1, \dots, \nod_k\} \in \Indeps{\forest}$.


\begin{itemize}
\item If $\forest = \nod_1$, then $k = 1$ (since the 
nodes are independent) and
$\prune{\forest}{s} \defined w[\fr{\forest}{\forest}]$.
Hence by Claim \gd{qui va bien} we have
that \gd{ça marche}.
\item Otherwise let $(\forest_1) \cdots (\forest_n) \defined \forest$.
For $1 \le j \le n$ we define $N_j \subseteq \{\nod_1, \dots, \nod_k\}$
for $1\le j \le n$ as the set of $\nod_i$ which
belong to $\forest_j$.
Then $ \biguplus_{1 \le j \le n} N_j = \{\nod_1, \dots, \nod_k\} $
and we set:
\begin{equation*}
\begin{aligned}
\prune{\forest}{\{\nod_1, \dots, \nod_k\}}
&\defined t(\forest_1) \cdots t(\forest_n) 
 \text{ where:} \\
&t: \forest_j  \mapsto
\left\{
    \begin{array}{l}
        \displaystyle \left(\prune{\forest_j}{N_j}\right) \tnorm{ if } N_j \neq \varnothing;\\
        \tnorm{ otherwise} \left\{
   				 \begin{array}{l}
       				  \mu(\forest_j) \tnorm{ if } N_{j{-1}} \neq \varnothing \text{ or } N_{j{+1}} \neq \varnothing;\\
      				  \vide \tnorm{ otherwise.}\\
  				  \end{array}
				\right. \\
    \end{array}
\right.
\end{aligned}
\end{equation*}
\end{itemize}









%%%%%% ARCHITECTURES ANCIENNE INDUCTION


\begin{sublemma} \label{slem:count-with-m}
Let $\ar = \tree{\ar_1} \cdots \tree{\ar_x} \tree{e} \tree{\Le} \tree{e} \tree{\ar'_1} \cdots \tree{\ar'_{x'}}$
where $x,x' \ge 0$. Then:
\begin{equation*}
\cou_{\ar}(\forest) = 
\left\{
    \begin{array}{l}
        0 \text{~~if~~} \forest \text{~~is not of the form}
	\tree{\gorest_1} \cdots \tree{\gorest_x}
        \tree{\forest_1} \cdots \tree{\forest_{n}} \tree{\gorest'_{1}} \cdots \tree{\gorest'_{x'}}\\
        \text{~~~with~~} n \ge 1 \text{~~and~~} \mu(\forest_1) = \mu(\forest_n) = e;\\
	\displaystyle \left(\prod_{i=1}^x
	\cou_{\ar_i}(\gorest_i)\right)  \times 
	 \left(\prod_{i=1}^{x'}
	\cou_{\ar_i}(\gorest'_i)\right) \times \cou_{\Le}(\tree{\forest_1} \cdots \tree{\forest_{n}})\\
	\text{~~~otherwise.}
    \end{array}
\right.
\end{equation*}
\end{sublemma}



\subsection{old}

Let $\displaystyle S(\forest) \defined  \Som_1 \cdots \Som_n
~\indic{\set{\nod^1_1, \dots, \nod^{n}_{r_{n}}} \in \Indep^{k}(\forest)}$.


\begin{equation*}
\begin{aligned}
 \\
& \Som_1 \cdots \Som_n~\indic{\{\nod^1_1, \dots, \nod^{n}_{r_n}\} \in \Indeps{\forest}}\\
 &= f'(\forest) \times
 \left( \Som_1 \cdots \Som_{n-1}~
 \indic{\set{\nod^1_1, \dots, \nod^{n-1}_{r_{n-1}}} \in \Indep^{k-r_n}(\forest)}
 \right) + f''(\forest)
 \end{aligned}
\end{equation*}

\begin{equation*}
\begin{aligned}
S(f) = &\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\set{\nod^{n}_1, \dots, \nod^{n}_{r_n}}\subseteq \itera{\forest}\\
\type{\forest}{\nod^n_{j}} = \tau_n}}
\indic{\{\nod^i_j : i,j\} \in \Indep^{k}(\forest)} \\
= &\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r} }}
\indic{\set{\nod^i_j : i,j } \in \Indep^{k}(\forest)} \\
= &\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r-1}}}
\sum_{\nod_{r-1} < \nod_{r}}\indic{\{\nod^1_1, \dots, \nod_{r}\} \in \Indep^{k}(\forest)} \\
= &\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r-1}}}
 \indic{\{\nod^1_1, \dots, \nod^n_{r-1}\} \in \Indep^{k-1}(\forest)}
\left(g_1+\sum_{\nod_{r-1} +3k < \nod_{r}} 1\right) \\
\end{aligned}
\end{equation*}
where $g_1 = 3k - \left| \left\{ \nod_r > \nod_{r-1} :
\{\nod^1_1, \dots, \nod^n_{r}\} \not\in \Indep^{k}(\forest) \right\}\right|$
which is positive since there are at most $3$ positions
forbidden for each.

Furthermore, the function 
\begin{equation*}
\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r-1}}}
 \indic{\{\nod^1_1, \dots, \nod^n_{r-1}\} \in \Indep^{k-1}(\forest)}
\left(g_1\right)
\end{equation*}
is polyregular (it suffices
to enumerate all independent nodes
with good types, check if the ordering
is respected and if they are not independent)
and clearly bounded by a polynomial of size $k-1$.
Hence we only have to treat the function:
\begin{equation*}
\begin{aligned}
&\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r-1}}}
 \indic{\{\nod^1_1, \dots, \nod^n_{r-1}\} \in \Indep^{k-1}(\forest)}
\sum_{\nod_{r-1} +3k < \nod_{r}} 1\\
& =\Som_1 \cdots \Som_{n-1}
 \sum_{\substack{\nod_1 < \cdots < \nod_{r-2}}}
  \sum_{\substack{\nod_{r-2} < \nod_{r-1}}}
 \indic{\{\nod^1_1, \dots, \nod^n_{r-1}\} \in \Indep^{k-1}(\forest)}
\sum_{\nod_{r-1} +3k < \nod_{r}} 1  \\
\end{aligned}
\end{equation*}





















The result is shown by induction on $k \ge 1$.

Let $\Le =: \multi{\tau_i \con r_1, \dots, \tau_n \con r_n}$
where $\tau_i = (m_i\cro{u_i}m'_i, d_i)$
and $(r_1, \dots, r_n) \in \Sigma_k$ and $r_i > 0$.
We assume that $d_1 \ge d_2 \ge  \dots \ge d_n$.
For $1 \le i \le n$, we 
denote:
\begin{equation*}
N_i(\forest) \defined
\left| \left\{\nod \in \itera{\forest}\cap \Nodes{\gorest} : \type{\forest}{\nod} = \tau_i \right\} \right|
\end{equation*}

\gd{blabla disjunction}
\subparagraph*{Case 1: $N_i(\forest) \ge 3({k{-}1})$ for all $1 \le i \le k$.}
We then define:
\begin{equation*}
\cou''_{\tree{\Le}} : \forest \mapsto \left(\prod_{i=1}^k N_i(\forest) {-} (i{-}1)\right)
\end{equation*}
This function is the Hadamard product of 
$k$ regular functions, hence it is polyblind.
Furthermore it is bounded by a polynomial of
degree $k$.

We now have to justify that $\cou''_{\tree{\Le}} \defined \cou_{\tree{\Le}} - \cou'_{\tree{\Le}} $
is non-negative, polyregular and bounded by a polynomial of degree $k{-}1$.

We note that:
\begin{equation*}
\begin{aligned}
\cou_{\tree{\Le}}(\forest) &=
\sum_{\substack{\nod_1 \le \dots \le \nod_{r_1} \in \Nodes{\gorest}\\
\forall 1\le i \le r_1,~\type{\forest}{\nod_i} = \tau_1 }}
\cdots
\sum_{\substack{\nod_1 \le \dots \le \nod_{r_n} \in \Nodes{\gorest}\\
\forall 1\le i \le r_n,~\type{\forest}{\nod_i} = \tau_n }}
\indic{\multi{\nod_1, \dots, \nod_k} \in \Indeps{\forest}}\\
&= \sum_{\substack{\nod_1 \le \dots \le \nod_{k-1} \in \Nodes{\gorest}\\
\forall 1\le i \le k,~\type{\forest}{\nod_i} = \tau_i }}
\indic{\multi{\nod_1, \dots, \nod_{k-1}} \in \Indeps{\forest}}\\
\end{aligned}
\end{equation*}


\subparagraph*{Case 2: $N_i(\forest) < 3({k{-}1})$ for some $1 \le i \le k$}.

In that case we define $\cou'_{\tree{\Le}}(\forest) = 0$ and
$\cou''_{\tree{\Le}}(\forest) = \cou'_{\tree{\Le}}(\forest)$.









The proof of this case is done using Sublemma \ref{slem:count-m}
 below.
 
\begin{sublemma} \label{slem:count-m}
Given $\tree{\Le} \in \Archs{\mu}{3|M|}{}$, one can build
two functions ${\cou'_{\tree{\Le}}},{\cou''_{\tree{\Le}}}: (\apar{A})^* \rightarrow \Nat$
such that $\cou_{\tree{\Le}} =  {\cou'_{\tree{\Le}}} +  {\cou''_{\tree{\Le}}}$ and:
\begin{itemize}
\item ${\cou'_{\tree{\Le}}}$ is polyblind and
has growth rate at most $k$;
\item  ${\cou''_{\tree{\Le}}}$ is polyregular and
has growth rate at most $k{-}1$.
\end{itemize}
\end{sublemma}
















\begin{definition}[Architecture]
Let $\forest \in \Facts{\mu}{}{w}$ and $\Nod \in \Indeps{\forest}$.
We define its \emph{architecture} by induction on $\forest$.
Since $\nod_1 \neq \forest$ we have
$\forest = \tree{\forest_1} \cdots \tree{\forest_n}$, then
for $1 \le i \le n$ we let $\Nod_i \defined \Nod \cap \Nodes{\forest_j}$ and:
\begin{itemize}
\item if  $n =2$ or $\Nod_j = \varnothing$ for all $1 \le j\le n$, we set:
\begin{equation*}
\begin{aligned}
\arch{\forest}{\set{\nod_1, \dots, \nod_k}} 
\defined (\arch{\forest_1}{\Nod_1}) \cdots  (\arch{\forest_{n}}{\Nod_{n}});\\
 \end{aligned}
\end{equation*}
\item otherwise $e \defined \mu(\forest_i)$ is idempotent.
Let $x+1$ (resp. $y{-}1$) be the smallest  (resp. largest) $1\le j\le n$
such that $\Nod_{j} = \varnothing$,
$\Le\defined \multi{(\lin{\forest}{\nod}, \depth{\forest}{\nod}): \nod \in \Nod_j \tnorm{ with } x < j < y}$ and:
\begin{equation*}
\begin{aligned}
&\arch{\forest}{\set{\nod_1, \dots, \nod_k}}\\
&\defined \tree{\arch{\forest_1}{\Nod_1}} \cdots  \tree{\arch{\forest_{x}}{\Nod_{x}}}\tree{e}\tree{\Le}\tree{e}
 \tree{\arch{\forest_{y}}{\Nod_{y}}} \cdots  \tree{\arch{\forest_{n}}{\Nod_n}}.\\
 \end{aligned}
\end{equation*}
\end{itemize}
\end{definition}

















\begin{lemma} \label{lem:lin-beaucoup} 
Let $\mu : A^* \rightarrow M$, $w \in A^*$, $\forest \in \Facts{\mu}{}{w}$. Let
 \mbox{$\Nod \in \Indep^{k}(\forest)$} and
\mbox{$p_0, \dots, p_{k} \in M$}, \mbox{$u_1, \dots, u_{k} \in A^+$} such that:
\begin{equation*}
\lin{\forest_i}{\Nod} = p_0 \left( \prod_{i=1}^{k} \cro{u_i} p_i \right).
\text{~~~Then~~~} \mu(\forest) = p_0 \left( \prod_{i=1}^{k} \mu(u_i) p_i \right)
\end{equation*}
and there exists a permutation $\tau$ of $\{1, \dots, k\}$ such that
for all $1 \le i \le \ell$:
\begin{equation*}
\lin{\forest}{\set{\nod_i}} = p_0 \left(\prod_{j=1}^{\tau(i)-1} \mu(u_j) p_{j}  \right)
\cro{u_\tau(i)} \left(\prod_{j=\tau(i)+1}^{\ell} p_{j-1} \mu(u_j)\right) p_{k}.
\end{equation*}
\end{lemma}

\begin{proof}
The proof is done by induction:
\begin{itemize}
\item if $k = 0$ the result is obvious;
\item if $\nod_1 = \forest$ (hence $k=1$), the result is obvious (use Remark \ref{rem:morphism-fr});
\item otherwise if $\forest = \tree{\forest_1} \cdots \tree{\forest_n}$, 
then for $1 \le j \le n$ we let $C_j \defined \set{\nod_1, \dots, \nod_k} \cap \Nodes{\forest_j}$
and we have
$
\lin{\forest}{\set{\nod_1, \dots, \nod_k}} = \lin{\forest_1}{C_1} \cdots  \lin{\forest_n}{C_n}
$.
By combining in this ordering the permutations obtained by induction,
we can build a suitable permutation $\tau$
since if $\nod_i \in C_j$ we have $\lin{\forest}{\set{\nod_i}}
= \mu(\forest_1) \dots \mu(\forest_{j-1}) \lin{\forest_j}{\set{\nod_j}} \mu(\forest_{j+1}) \cdots \mu(\forest_{n})$.
\end{itemize}
\vspace*{-1\baselineskip}
\end{proof}





